Enhancing LLMs for Governance with Human Oversight: Evaluating and Aligning LLMs on Expert Classification of Climate Misinformation for Detecting False or Misleading Claims about Climate Change

Climate misinformation is a problem that has the potential to be substantially aggravated by the development of Large Language Models (LLMs). In this study we evaluate the potential for LLMs to be part of the solution for mitigating online dis/misinformation rather than the problem. Employing a public expert annotated dataset and a curated sample of social media content we evaluate the performance of proprietary vs. open source LLMs on climate misinformation classification task, comparing them to existing climate-focused computer-assisted tools and expert assessments. Results show (1) open-source models substantially under-perform in classifying climate misinformation compared to proprietary models, (2) existing climate-focused computer-assisted tools leveraging expert-annotated datasets continues to outperform many of proprietary models, including GPT-4o, and (3) demonstrate the efficacy and generalizability of fine-tuning GPT-3.5-turbo on expert annotated dataset in classifying claims about climate change at the equivalency of climate change experts with over 20 years of experience in climate communication. These findings highlight 1) the importance of incorporating human-oversight, such as incorporating expert-annotated datasets in training LLMs, for governance tasks that require subject-matter expertise like classifying climate misinformation, and 2) the potential for LLMs in facilitating civil society organizations to engage in various governance tasks such as classifying false or misleading claims in domains beyond climate change such as politics and health science.

==> Makefile <==
# LATEX: pdflatex | xelatex | lualatex
LATEX = lualatex
LATEX_FLAGS = -shell-escape
BIBTEX = bibtex

FILES = $(patsubst %.tex, %.pdf, $(wildcard *.tex))

all: $(FILES)


%.pdf: %.tex
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	-$(BIBTEX) `basename $< .tex`
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	qpdf --linearize --newline-before-endstream $@ /tmp/$@
	mv /tmp/$@ $@

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,cut,abs,xmpi,xmpdata,*~}
	-rm -rf out _minted* auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done
	-rm $(FILES)

cleanall: clean
	-rm -rf out auto

==> abstract.tex <==
Climate misinformation is a problem that has the potential to be substantially aggravated by the development of Large Language Models (LLMs). In this study we evaluate the potential for LLMs to be part of the solution for mitigating online dis/misinformation rather than the problem. Employing a public expert annotated dataset and a curated sample of social media content we evaluate the performance of proprietary vs. open source LLMs on climate misinformation classification task, comparing them to existing climate-focused computer-assisted tools and expert assessments. Results show (1) state-of-the-art (SOTA) open-source models substantially under-perform in classifying climate misinformation compared to proprietary models, (2) existing climate-focused computer-assisted tools  leveraging expert-annotated datasets continues to outperform many of proprietary models, including GPT-4o, and (3) demonstrate the efficacy and generalizability of fine-tuning GPT-3.5-turbo on expert annotated dataset in classifying claims about climate change at the equivalency of climate change experts with over 20 years of experience in climate communication. These findings highlight 1) the importance of incorporating human-oversight, such as incorporating expert-annotated datasets in training LLMs, for governance tasks that require subject-matter expertise like classifying climate misinformation, and 2) the potential for LLMs in facilitating civil society organizations to engage in various governance tasks such as classifying false or misleading claims in domains beyond climate change such as politics and health science.

==> prompts.tex <==
\begin{document}
\begin{verbatim}
    system_instruction="""
Overview:
---------
CARDS: Computer Assisted Recognition of Denial and Skepticism, is a machine learning project. Our
aim is to train a computer to automatically detect and categorize misinformation about climate change.
The end goal is that a computer can look at some text and successfully identify any climate
misinformation - and even identify specific denialist claims. If successful, this will enable us to travel
back in time and build a history of climate misinformation, including when myths originated and how
they’ve evolved over time. It will also enable us to spot new publishing of denialist claims in real-time.

Context:
--------
Use the following coding rubric to answer the task assigned to you:
[
  {
    "code": "1",
    "identifier": 1,
    "claim": "Global warming is not happening"
  },
  {
    "code": "1.1",
    "identifier": 6,
    "claim": "Ice/permafrost/snow cover isn't melting"
  },
  {
    "code": "1.1.1",
    "identifier": 7,
    "claim": "Antarctica is gaining ice/not warming"
  },
  {
    "code": "1.1.2",
    "identifier": 8,
    "claim": "Greenland is gaining ice/not melting"
  },
  {
    "code": "1.1.3",
    "identifier": 9,
    "claim": "Arctic sea ice isn't vanishing"
  },
  {
    "code": "1.1.4",
    "identifier": 10,
    "claim": "Glaciers aren't vanishing"
  },
  {
    "code": "1.2",
    "identifier": 11,
    "claim": "We're heading into an ice age/global cooling"
  },
  {
    "code": "1.3",
    "identifier": 12,
    "claim": "Weather is cold/snowing"
  },
  {
    "code": "1.4",
    "identifier": 13,
    "claim": "Climate hasn't warmed/changed over the last (few) decade(s)"
  },
  {
    "code": "1.5",
    "identifier": 14,
    "claim": "Oceans are cooling/not warming"
  },
  {
    "code": "1.6",
    "identifier": 15,
    "claim": "Sea level rise is exaggerated/not accelerating"
  },
  {
    "code": "1.7",
    "identifier": 16,
    "claim": "Extreme weather isn't increasing/has happened before/isn't linked to climate change"
  },
  {
    "code": "1.8",
    "identifier": 17,
    "claim": "They changed the name from global warming' to climate change\u2019"
  },
  {
    "code": "2",
    "identifier": 2,
    "claim": "Human greenhouse gases are not causing climate change"
  },
  {
    "code": "2.1",
    "identifier": 18,
    "claim": "It's natural cycles/variation"
  },
  {
    "code": "2.1.1",
    "identifier": 19,
    "claim": "It's the sun/cosmic rays/astronomical"
  },
  {
    "code": "2.1.2",
    "identifier": 20,
    "claim": "It's geological (includes volcanoes)"
  },
  {
    "code": "2.1.3",
    "identifier": 21,
    "claim": "It's the ocean/internal variability"
  },
  {
    "code": "2.1.4",
    "identifier": 22,
    "claim": "Climate has changed naturally/been warm in the past"
  },
  {
    "code": "2.1.5",
    "identifier": 23,
    "claim": "Human CO2 emissions are tiny compared to natural CO2 emission"
  },
  {
    "code": "2.2",
    "identifier": 24,
    "claim": "It's non-greenhouse gas human climate forcings (aerosols, land use)"
  },
  {
    "code": "2.3",
    "identifier": 25,
    "claim": "There's no evidence for greenhouse effect/carbon dioxide driving climate change"
  },
  {
    "code": "2.3.1",
    "identifier": 26,
    "claim": "Carbon dioxide is just a trace gas"
  },
  {
    "code": "2.3.2",
    "identifier": 27,
    "claim": "Greenhouse effect is saturated/logarithmic"
  },
  {
    "code": "2.3.3",
    "identifier": 28,
    "claim": "Carbon dioxide lags/not correlated with climate change"
  },
  {
    "code": "2.3.4",
    "identifier": 29,
    "claim": "Water vapor is the most powerful greenhouse gas"
  },
  {
    "code": "2.3.5",
    "identifier": 30,
    "claim": "There's no tropospheric hot spot"
  },
  {
    "code": "2.3.6",
    "identifier": 75,
    "claim": "CO2 was higher in the past"
  },
  {
    "code": "2.4",
    "identifier": 76,
    "claim": "C02 is not rising/ocean pH is not falling"
  },
  {
    "code": "2.5",
    "identifier": 78,
    "claim": "Human CO2 emissions are miniscule/not raising atmospheric CO2"
  },
  {
    "code": "3",
    "identifier": 3,
    "claim": "Climate impacts/global warming is beneficial/not bad"
  },
  {
    "code": "3.1",
    "identifier": 31,
    "claim": "Climate sensitivity is low/negative feedbacks reduce warming"
  },
  {
    "code": "3.2",
    "identifier": 32,
    "claim": "Species/plants/reefs aren't showing climate impacts yet/are benefiting from climate"
  },
  {
    "code": "3.2.1",
    "identifier": 33,
    "claim": "Species can adapt to global warming"
  },
  {
    "code": "3.2.2",
    "identifier": 34,
    "claim": "Polar bears are not in danger from climate change"
  },
  {
    "code": "3.2.3",
    "identifier": 77,
    "claim": "Ocean acidification/coral impacts aren't serious"
  },
  {
    "code": "3.3",
    "identifier": 35,
    "claim": "C02 is beneficial/not a pollutant"
  },
  {
    "code": "3.3.1",
    "identifier": 36,
    "claim": "CO2 is plant food"
  },
  {
    "code": "3.4",
    "identifier": 37,
    "claim": "It's only a few degrees (or less)"
  },
  {
    "code": "3.5",
    "identifier": 38,
    "claim": "Climate change does not contribute to human conflict/threaten national security"
  },
  {
    "code": "3.6",
    "identifier": 39,
    "claim": "Climate change doesn't negatively impact health"
  },
  {
    "code": "4",
    "identifier": 4,
    "claim": "Climate solutions won't work"
  },
  {
    "code": "4.1",
    "identifier": 40,
    "claim": "Climate policies (mitigation or adaptation) are harmful"
  },
  {
    "code": "4.1.1",
    "identifier": 41,
    "claim": "Climate policy will increase costs/harm economy/kill jobs"
  },
  {
    "code": "4.1.2",
    "identifier": 42,
    "claim": "Proposed action would weaken national security/national sovereignty/cause conflict"
  },
  {
    "code": "4.1.3",
    "identifier": 43,
    "claim": "Proposed action would actually harm the environment and species"
  },
  {
    "code": "4.1.4",
    "identifier": 44,
    "claim": "Future generations will be richer and better able to adapt"
  },
  {
    "code": "4.1.5",
    "identifier": 45,
    "claim": "Climate policy limits liberty/freedom/capitalism"
  },
  {
    "code": "4.2",
    "identifier": 46,
    "claim": "Climate policies are ineffective/flawed"
  },
  {
    "code": "4.2.1",
    "identifier": 47,
    "claim": "Clean energy/green jobs/businesses won't work"
  },
  {
    "code": "4.2.2",
    "identifier": 48,
    "claim": "Markets/private sector are economically more efficient than government policies"
  },
  {
    "code": "4.2.3",
    "identifier": 49,
    "claim": "Climate policy will make negligible difference to climate change"
  },
  {
    "code": "4.2.4",
    "identifier": 50,
    "claim": "A single country/region only contributes a small % of global emissions"
  },
  {
    "code": "4.2.5",
    "identifier": 51,
    "claim": "Better to adapt/geoengineer/increase resiliency"
  },
  {
    "code": "4.2.6",
    "identifier": 52,
    "claim": "Climate action is pointless because of China/India/other countries' emissions"
  },
  {
    "code": "4.2.7",
    "identifier": 80,
    "claim": "We should invest in technology/reduce poverty/disease first"
  },
  {
    "code": "4.3",
    "identifier": 53,
    "claim": "It's too hard to solve"
  },
  {
    "code": "4.3.1",
    "identifier": 54,
    "claim": "Climate policy is politically/legally/economically/technically too difficult"
  },
  {
    "code": "4.3.2",
    "identifier": 79,
    "claim": "Media/public support/acceptance is low/decreasing"
  },
  {
    "code": "4.4",
    "identifier": 55,
    "claim": "Clean energy technology/biofuels won't work"
  },
  {
    "code": "4.4.1",
    "identifier": 56,
    "claim": "Clean energy/biofuels are too expensive/unreliable/counterproductive/harmful"
  },
  {
    "code": "4.4.2",
    "identifier": 57,
    "claim": "Carbon Capture & Sequestration (CCS) is unproven/expensive"
  },
  {
    "code": "4.5",
    "identifier": 58,
    "claim": "People need energy (e.g., from fossil fuels/nuclear)"
  },
  {
    "code": "4.5.1",
    "identifier": 81,
    "claim": "Fossil fuel reserves are plentiful"
  },
  {
    "code": "4.5.2",
    "identifier": 82,
    "claim": "Fossil fuels are cheap/good/safe for society/economy/environment"
  },
  {
    "code": "4.5.3",
    "identifier": 83,
    "claim": "Nuclear power is safe/good for society/economy/environment"
  },
  {
    "code": "5",
    "identifier": 5,
    "claim": "Climate movement/science is unreliable"
  },
  {
    "code": "5.1",
    "identifier": 59,
    "claim": "Climate-related science is uncertain/unsound/unreliable (data, methods & models)"
  },
  {
    "code": "5.1.1",
    "identifier": 60,
    "claim": "There's no scientific consensus on climate/the science isn't settled"
  },
  {
    "code": "5.1.2",
    "identifier": 61,
    "claim": "Proxy data is unreliable (includes hockey stick)"
  },
  {
    "code": "5.1.3",
    "identifier": 62,
    "claim": "Temperature record is unreliable"
  },
  {
    "code": "5.1.4",
    "identifier": 63,
    "claim": "Models are wrong/unreliable/uncertain"
  },
  {
    "code": "5.2",
    "identifier": 64,
    "claim": "Climate movement is alarmist/wrong/political/biased/hypocritical (people or groups)"
  },
  {
    "code": "5.2.1",
    "identifier": 65,
    "claim": "Climate movement is religion"
  },
  {
    "code": "5.2.2",
    "identifier": 66,
    "claim": "Media (including bloggers) is alarmist/wrong/political/biased"
  },
  {
    "code": "5.2.3",
    "identifier": 67,
    "claim": "Politicians/government/UN are alarmist/wrong/political/biased"
  },
  {
    "code": "5.2.4",
    "identifier": 68,
    "claim": "Environmentalists are alarmist/wrong/political/biased"
  },
  {
    "code": "5.2.5",
    "identifier": 69,
    "claim": "Scientists/academics are alarmist/wrong/political/biased"
  },
  {
    "code": "5.3",
    "identifier": 70,
    "claim": "Climate change (science or policy) is a conspiracy (deception)"
  },
  {
    "code": "5.3.1",
    "identifier": 71,
    "claim": "Climate policy/renewables is a hoax/scam/conspiracy/secretive"
  },
  {
    "code": "5.3.2",
    "identifier": 72,
    "claim": "Climate science is a hoax/scam/conspiracy/secretive/money-motivated"
  }
]

Task:
-----
Classify whether a text excerpt belong to one of the claims outlined in the Context section provided in JSON format. Only respond in a JSON  format outlined below and don't make things up beyond what is given to you in the context. Below is the formatted JSON response template:
{
  "code": "CODE",
  "identifier": IDENTIFIER,
  "claim": "CLAIM"
}

If no claim is present in the text, just return a formatted json response like this one:
{
  "code": "0",
  "identifier": 0,
  "claim": "no claim"
}


This the end of the instructions. Now you will be provided a question with an excerpt of text and asked to identify the claim to which it belongs to.
"""


\end{verbatim}
\end{document}

==> table-gpt3.5-vs-cards-sm-data.tex <==
\renewcommand{\arraystretch}{1.5} % Adjust row height spacing
\begin{table*}[ht]
\small
\centering
\begin{tabularx}{\textwidth}{>{\raggedright\arraybackslash}p{4.5cm}>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}Xc>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X>{\centering\arraybackslash}X}
\hline
 & \multicolumn{4}{c}{\textbf{Fine-tuned GPT-3.5-turbo}} & & \multicolumn{4}{c}{\textbf{RoBERTa$_{\mathit{large}}$}} \\
\cline{2-5} \cline{7-10}
 \textbf{Claim Code} & \textbf{Precision} & \textbf{Recall} & \textbf{F1} & \textbf{Support} & & \textbf{Precision} & \textbf{Recall} & \textbf{F1} & \textbf{Support} \\
\hline
0 (No claim) & 0.94 & 0.94 & 0.94 & 491 & & 0.76 & 0.96 & 0.85 & 491 \\
1 (Global warming is not happening) & 0.71 & 1.00 & 0.83 & 24 & & 0.71 & 0.62 & 0.67 & 24 \\
2 (Humans' greenhouse gases are not causing global warming) & 0.93 & 0.93 & 0.93 & 14 & & 1.00 & 0.79 & 0.88 & 14 \\
3 (Climate impacts are not bad) & 0.57 & 1.00 & 0.73 & 8 & & 0.57 & 0.50 & 0.53 & 8 \\
4 (Climate solutions won’t work) & 0.95 & 0.94 & 0.95 & 274 & & 0.93 & 0.63 & 0.75 & 274 \\
5 (The climate movement and/or science are unreliable) & 0.99 & 0.89 & 0.94 & 103 & & 0.90 & 0.62 & 0.74 & 103 \\
\hline
\textbf{Accuracy} &  &  & 0.94 & 914 & &  &  & 0.81 & 914 \\
\textbf{Macro avg} & 0.85 & 0.95 & 0.88 & 914 & & 0.81 & 0.69 & 0.74 & 914 \\
\textbf{Weighted avg} & 0.94 & 0.94 & 0.94 & 914 & & 0.83 & 0.81 & 0.80 & 914 \\
\hline
\end{tabularx}
\caption{Performance comparison between fine-tuned GPT-3.5-turbo and RoBERTa$_{\mathit{large}}$ on the social media dataset across the five categories of super-claims.}
\label{tab:performance}
\end{table*}


==> table-model-performance-by-super-claim.tex <==
\begin{table}[h]
\centering
\caption{Performance comparison of various models. -- 0 claim}
\label{tab:model_performance}
\begin{tabular}{lcccc}
\toprule
\textbf{Model} & \textbf{Precision} & \textbf{Recall} & \textbf{F1-Score} & \textbf{Support} \\
\midrule
CARDS-model & 0.90 & 0.95 & 0.93 & 1754 \\
fine-tuned-GPT-3.5-Turbo & 0.8907 & 0.9567 & 0.9225 & 1754 \\
fine-tuned-GPT-4o & 0.87 & 0.97 & 0.92 & 1754 \\
GPT-4 & 0.94 & 0.73 & 0.83 & 1754 \\
GPT-4o & 0.97 & 0.71 & 0.82 & 1754 \\
GPT-4o-mini & 0.97 & 0.71 & 0.82 & 1754 \\
Gemini-1.5-flash & 0.97 & 0.56 & 0.71 & 1754 \\
GPT-3.5-zero-shot & 0.97 & 0.36 & 0.53 & 1754 \\
llama-3-8b-instruct & 0.97 & 0.17 & 0.28 & 1754 \\
llama2-7b & 0.60 & 0.15 & 0.23 & 1754 \\
gemma-2-2b & 0.64 & 0.13 & 0.21 & 1754 \\
llama3-8b-completion & 0.83 & 0.09 & 0.16 & 1754 \\
Mistral-7B-v0.8-instruct & 0.97 & 0.07 & 0.13 & 1754 \\
llama3.1-8b & 0.60 & 0.03 & 0.06 & 1754 \\
Phi-3.5-3.8b & 0.80 & 0.03 & 0.05 & 1754 \\
llama2-7b-chat & 0.68 & 0.01 & 0.02 & 1754 \\
llama3.1-instruct-8b & 0.56 & 0.00 & 0.01 & 1754 \\
Mistral-7B-v0.3 & 0.00 & 0.00 & 0.00 & 1754 \\
gemma-2-9b & 0.33 & 0.00 & 0.00 & 1754 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[h]
\centering
\caption{Performance comparison of various models -- claim 1}
\label{tab:model_performance_2}
\begin{tabular}{lcccc}
\toprule
\textbf{Model} & \textbf{Precision} & \textbf{Recall} & \textbf{F1-Score} & \textbf{Support} \\
\midrule
fine-tuned-GPT-4o & 0.91 & 0.86 & 0.88 & 262 \\
fine-tuned-GPT-3.5-Turbo & 0.9024 & 0.8506 & 0.8757 & 262 \\
CARDS-model & 0.92 & 0.80 & 0.86 & 262 \\
GPT-4o & 0.70 & 0.83 & 0.76 & 262 \\
GPT-4o-mini & 0.70 & 0.83 & 0.76 & 262 \\
GPT-4 & 0.69 & 0.84 & 0.76 & 262 \\
Gemini-1.5-flash & 0.60 & 0.82 & 0.69 & 262 \\
GPT-3.5-zero-shot & 0.42 & 0.92 & 0.57 & 262 \\
Phi-3.5-3.8b & 0.58 & 0.53 & 0.55 & 262 \\
llama3.1-instruct-8b & 0.35 & 0.68 & 0.46 & 262 \\
llama-3-8b-instruct & 0.30 & 0.87 & 0.45 & 262 \\
Mistral-7B-v0.8-instruct & 0.24 & 0.98 & 0.38 & 262 \\
llama3-8b-completion & 0.12 & 0.80 & 0.21 & 262 \\
gemma-2-9b & 0.10 & 1.00 & 0.19 & 262 \\
llama3.1-8b & 0.10 & 0.74 & 0.18 & 262 \\
Mistral-7B-v0.4 & 0.09 & 1.00 & 0.17 & 262 \\
llama2-7b-chat & 0.09 & 0.90 & 0.16 & 262 \\
gemma-2-2b & 0.09 & 0.74 & 0.16 & 262 \\
llama2-7b & 0.08 & 0.34 & 0.13 & 262 \\
\bottomrule
\end{tabular}
\end{table}


\begin{table}[h]
\centering
\caption{Performance comparison of various models -- claims 2.}
\label{tab:model_performance_3}
\begin{tabular}{lcccc}
\toprule
\textbf{Model} & \textbf{Precision} & \textbf{Recall} & \textbf{F1-Score} & \textbf{Support} \\
\midrule
fine-tuned-GPT-4o & 0.91 & 0.85 & 0.88 & 172 \\
fine-tuned-GPT-3.5-Turbo & 0.8889 & 0.8372 & 0.8623 & 172 \\
CARDS-model & 0.82 & 0.88 & 0.85 & 172 \\
GPT-4o & 0.67 & 0.94 & 0.78 & 172 \\
GPT-4o-mini & 0.67 & 0.94 & 0.78 & 172 \\
GPT-4 & 0.72 & 0.80 & 0.76 & 172 \\
Gemini-1.5-flash & 0.60 & 0.83 & 0.69 & 172 \\
GPT-3.5-zero-shot & 0.51 & 0.58 & 0.54 & 172 \\
llama-3-8b-instruct & 0.27 & 0.16 & 0.20 & 172 \\
Mistral-7B-v0.8-instruct & 0.13 & 0.15 & 0.14 & 172 \\
llama3.1-8b & 0.08 & 0.08 & 0.08 & 172 \\
llama3.1-instruct-8b & 0.05 & 0.11 & 0.07 & 172 \\
llama2-7b & 0.04 & 0.05 & 0.04 & 172 \\
llama2-7b-chat & 0.08 & 0.02 & 0.04 & 172 \\
llama3-8b-completion & 0.05 & 0.02 & 0.03 & 172 \\
gemma-2-2b & 0.06 & 0.02 & 0.03 & 172 \\
Phi-3.5-3.8b & 0.02 & 0.01 & 0.02 & 172 \\
Mistral-7B-v0.5 & 0.00 & 0.00 & 0.00 & 172 \\
gemma-2-9b & 0.00 & 0.00 & 0.00 & 172 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[h]
\centering
\caption{Performance comparison of various models. -- claims 3.}
\label{tab:model_performance_4}
\begin{tabular}{lcccc}
\toprule
\textbf{Model} & \textbf{Precision} & \textbf{Recall} & \textbf{F1-Score} & \textbf{Support} \\
\midrule
fine-tuned-GPT-4o & 0.92 & 0.92 & 0.92 & 121 \\
CARDS-model & 0.91 & 0.92 & 0.91 & 121 \\
fine-tuned-GPT-3.5-Turbo & 0.9060 & 0.8760 & 0.8908 & 121 \\
GPT-4 & 0.77 & 0.89 & 0.83 & 121 \\
GPT-4o & 0.78 & 0.84 & 0.81 & 121 \\
GPT-4o-mini & 0.78 & 0.84 & 0.81 & 121 \\
Gemini-1.5-flash & 0.75 & 0.78 & 0.76 & 121 \\
GPT-3.5-zero-shot & 0.41 & 0.83 & 0.55 & 121 \\
llama-3-8b-instruct & 0.37 & 0.57 & 0.45 & 121 \\
Mistral-7B-v0.8-instruct & 0.25 & 0.77 & 0.38 & 121 \\
Phi-3.5-3.8b & 0.77 & 0.25 & 0.38 & 121 \\
gemma-2-9b & 0.53 & 0.27 & 0.36 & 121 \\
llama3.1-instruct-8b & 0.24 & 0.61 & 0.34 & 121 \\
llama3-8b-completion & 0.17 & 0.23 & 0.19 & 121 \\
llama2-7b-chat & 0.13 & 0.08 & 0.10 & 121 \\
llama3.1-8b & 0.07 & 0.13 & 0.09 & 121 \\
Mistral-7B-v0.6 & 1.00 & 0.04 & 0.08 & 121 \\
llama2-7b & 0.04 & 0.14 & 0.06 & 121 \\
gemma-2-2b & 0.05 & 0.05 & 0.05 & 121 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[h]
\centering
\caption{Performance comparison of various models. -- claim 4.}
\label{tab:model_performance_5}
\begin{tabular}{lcccc}
\toprule
\textbf{Model} & \textbf{Precision} & \textbf{Recall} & \textbf{F1-Score} & \textbf{Support} \\
\midrule
CARDS-model & 0.86 & 0.64 & 0.74 & 173 \\
fine-tuned-GPT-3.5-Turbo & 0.8271 & 0.6358 & 0.7190 & 173 \\
fine-tuned-GPT-4o & 0.86 & 0.48 & 0.61 & 173 \\
GPT-4o & 0.48 & 0.87 & 0.61 & 173 \\
GPT-4o-mini & 0.48 & 0.87 & 0.61 & 173 \\
GPT-4 & 0.46 & 0.85 & 0.60 & 173 \\
Gemini-1.5-flash & 0.33 & 0.91 & 0.49 & 173 \\
GPT-3.5-zero-shot & 0.31 & 0.82 & 0.46 & 173 \\
llama-3-8b-instruct & 0.23 & 0.78 & 0.36 & 173 \\
Mistral-7B-v0.8-instruct & 0.19 & 0.81 & 0.31 & 173 \\
llama3.1-instruct-8b & 0.28 & 0.31 & 0.29 & 173 \\
gemma-2-9b & 0.29 & 0.19 & 0.23 & 173 \\
llama3-8b-completion & 0.14 & 0.42 & 0.21 & 173 \\
llama3.1-8b & 0.08 & 0.17 & 0.11 & 173 \\
llama2-7b & 0.08 & 0.22 & 0.11 & 173 \\
Phi-3.5-3.8b & 0.67 & 0.06 & 0.11 & 173 \\
gemma-2-2b & 0.05 & 0.04 & 0.05 & 173 \\
llama2-7b-chat & 0.04 & 0.02 & 0.03 & 173 \\
Mistral-7B-v0.7 & 0.33 & 0.01 & 0.01 & 173 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[h]
\centering
\caption{Performance comparison of various models. -- claims 5}
\label{tab:model_performance_6}
\begin{tabular}{lcccc}
\toprule
\textbf{Model} & \textbf{Precision} & \textbf{Recall} & \textbf{F1-Score} & \textbf{Support} \\
\midrule
CARDS-model & 0.82 & 0.75 & 0.78 & 422 \\
fine-tuned-GPT-3.5-Turbo & 0.8421 & 0.7204 & 0.7765 & 422 \\
fine-tuned-GPT-4o & 0.87 & 0.65 & 0.74 & 422 \\
GPT-4o & 0.59 & 0.86 & 0.70 & 422 \\
GPT-4o-mini & 0.59 & 0.86 & 0.70 & 422 \\
GPT-4 & 0.60 & 0.81 & 0.69 & 422 \\
Gemini-1.5-flash & 0.52 & 0.86 & 0.65 & 422 \\
GPT-3.5-zero-shot & 0.39 & 0.72 & 0.50 & 422 \\
llama-3-8b-instruct & 0.29 & 0.68 & 0.41 & 422 \\
Mistral-7B-v0.8-instruct & 0.38 & 0.35 & 0.37 & 422 \\
llama3.1-instruct-8b & 0.20 & 0.72 & 0.32 & 422 \\
Phi-3.5-3.8b & 0.17 & 0.97 & 0.28 & 422 \\
llama3-8b-completion & 0.36 & 0.19 & 0.25 & 422 \\
gemma-2-9b & 0.41 & 0.15 & 0.22 & 422 \\
llama2-7b & 0.13 & 0.08 & 0.10 & 422 \\
llama3.1-8b & 0.15 & 0.06 & 0.08 & 422 \\
gemma-2-2b & 0.11 & 0.03 & 0.04 & 422 \\
llama2-7b-chat & 0.19 & 0.02 & 0.03 & 422 \\
Mistral-7B-v0.8 & 0.00 & 0.00 & 0.00 & 422 \\
\bottomrule
\end{tabular}
\end{table}


==> table-refusal-from-llm-on-cards-dataset.tex <==
\subsection{Examples of LLMs refusing to classify claims}
Description


\begingroup
\setlength\LTleft{0pt} % Align longtable to the left margin
\setlength\LTright{0pt} % Align longtable to the right margin
\begin{longtable}{p{7cm}p{4cm}p{3cm} >{\centering\arraybackslash}p{1.5cm} >{\centering\arraybackslash}p{1.5cm}}
  \toprule
  Paragraph & Expert Annotation & Model & Response \\
  \midrule
  \endfirsthead
  \toprule
  Paragraph & Expert Annotation & Model & Response \\
  \midrule
  \endhead
  \bottomrule
  \endfoot

  Nuccitellis answer to this unexceptionable and temperately-expressed statement is that sea level rises chiefly through thermal expansion and melting land ice, so it is all our fault. However, it ought to have been obvious even to Nuccitelli thermal expansion and land-ice melt happen whether Man or nature is the cause. & 2\_1 & Llama3.1-8B & I'm not sure if this is the right place to post this,but I\'m trying to get a better.\\
  \\
  Grafting instrumental data onto proxy data to produce a seemingly continuous record is trickery, because instrumental data, unlike proxy data, are massively influenced by land-use changes and site-specific quality control issues. & 5\_2 & Llama3.1-8B & I'm not sure if this is the right place to post this, but I\'m trying to get a better.\\
  \\
  The scientists begin their article noting that Growth of plants under elevated CO2 frequently leads to increased growth rates, but that was not the focus of their study. Many others have grown tobacco in elevated CO2 and confirmed that tobacco, like virtually every other plant in the world, benefits from higher concentrations of CO2. Matros et al. made a series of measurements on how elevated CO2 impacts nicotine, and they conclude that Cultivation of tobacco plants at elevated CO2 leads to a marked decrease of nicotine, the major nitrogen-rich secondary metabolite in tobacco at lower nitrogen supply and At higher nitrogen supply, nicotine content was not further influenced by CO2. See, if you are trying to quit smoking, elevated CO2 is your friend and it generally acts to lower the nicotine level of the plants! & 3\_3 & Gemini & harmful content\\
  \\
  Sprawling wind and solar installations and transmission lines across millions of acres of wildlife and scenic areas will kill millions of eagles, hawks, and other birds and bats. & 4\_1 & Gemini & harmful content\\
  \\
  and since the cost of AB 32 (direct \& indirect) is at least \$116 Billion, the cost to "avoid global warming" per 1 C would be \$116,000,000,000/.000087429 = \$1,326,790,881,744,043 (\$1.3 Quadrillion per degree). Note: Global GDP (61.1 trillion) is less than 5\% of this amount. Looks like the cost/(assumed benefits) ratio is rather high, even if you are a true believer.& 4\_1 & Gemini & harmful content\\
  \\
  mostly find Earth Day just plain annoying for the rank hypocrisy on display. A state-sponsored religious day of worship, along with all of the 1st Amendment-violating regulations to codify it.& 5\_2 & Gemini & harmful content \\
  \\
  We see below how many of the UWA hosts benefit from climate change grants, and thus would potentially gain from promoting a baseless smear against critics who threaten their funding or status. These hypocrites are happy to promote the untruth that skeptics are funded to speak, when the they themselves are the ones who benefit financially from a dubious scare campaign. The professors-at-large program is supposed to foster public debate, but four of the ten Oreskes hosts signed a letter seeking to silence a skeptic from speaking at another university. & 5\_2 & Gemini & harmful content\\
  \\
  It will likely be open season on Mann. Anyone may now freely dismiss him in the harshest terms as a junk scientist who shilled for a failed global warming cabal. Without fear of his civil legal redress, we may now refer to Mann for what he is: a climate criminal, a fraudster.& 5\_2 & Gemini & harmful content.
\end{longtable}
\endgroup

